Multi-objective optimization of the magnetic wiping process in dip-coating

Electromagnetic wiping systems allow to pre-meter the coating thickness of the liquid metal on a moving substrate. These systems have the potential to provide a more uniform coating and significantly higher production rates compared to pneumatic wiping, but they require substantially larger amounts of energy. This work presents a multi-objective optimization accounting for (1) maximal wiping efficiency (2) maximal smoothness of the wiping meniscus, and (3) minimal Joule heating. We present the Pareto front, identifying the best wiping conditions given a set of weights for the three competing objectives. The optimization was based on a 1D steady-state integral model, whose prediction scales according to the Hartmann number (Ha). The optimization uses a multi-gradient approach, with gradients computed with a combination of finite differences and variational methods. The results show that the wiping efficiency depends solely on Ha and not the magnetic field distribution. Moreover, we show that the liquid thickness becomes insensitive to the intensity of the magnetic field above a certain threshold and that the current distribution (hence the Joule heating) is mildly affected by the magnetic field's intensity and shape.

==> Figures/curvature_sensitivity_validation.tex <==
\begin{table*}[!htbp]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.3\linewidth]{Pictures/appendix/validation_curvature_grad/validation_curv_grad_Ha_eps_1.png} &         \includegraphics[width=0.3\linewidth]{Pictures/appendix/validation_curvature_grad/validation_curv_grad_Ha_eps_10.png}
    \end{tabular}
    \caption{Validation curvature sensitivity}
    \label{fig:myfig1}
\end{table*}

==> Figures/curvature_vs_Ha_epsilon.tex <==
\begin{figure}[h]
\centering
% For eps or pdf graphics
\includegraphics[width=0.5\textwidth]{Pictures/curvature_vs_Ha_epsilon.png}\quad
%  \raisebox{1.3in}{a)}\input{figa}\quad
%  \raisebox{1.3in}{b)}\input{figb}
\caption{Plot of the curvature ($J_2$) as a function of the Hartmann number ($H_a$) and the magnetic field standard deviation ($\gamma$)}
\label{curvature_vs_Ha_epsilon}
\end{figure}

==> Figures/hump_formation.tex <==
\begin{figure}[h!]
\centering
% For eps or pdf graphics
\includegraphics[width=0.457\textwidth]{Pictures/current_density_44.png}
\vspace{-.5cm}
%  \raisebox{1.3in}{a)}\input{figa}\quad
%  \raisebox{1.3in}{b)}\input{figb}
\caption{\small Examples of steady state solution for different intensities of the magnetic fields, scaled in terms of Hartman number $H_{a} = (\sigma[B]^2U_p/\rho g)^{1/2}$, with $[B]$ the maximum intensity of the magnetic field, $g$ the gravity acceleration(from left to right) and $\sigma$ the electrical conductivity. On the right, the high $H_{a}$ results in a solitary hump in the run-back flow, $H_a = 3$ (left) and $H_a = 10$ (right).}
\label{hump_formation}
\end{figure}

\begin{figure}[h!]
\centering
% For eps or pdf graphics
\includegraphics[width=0.457\textwidth]{Pictures/current_density.png}
%  \raisebox{1.3in}{a)}\input{figa}\quad
%  \raisebox{1.3in}{b)}\input{figb}
\caption{\small Examples of steady state solution for different intensities of the magnetic fields, scaled in terms of Hartman number $H_{a} = (\sigma[B]^2U_p/\rho g)^{1/2}$, with $[B]$ the maximum intensity of the magnetic field, $g$ the gravity acceleration(from left to right) and $\sigma$ the electrical conductivity. On the right, the high $H_{a}$ results in a solitary hump in the run-back flow, $H_a = 3$ (left) and $H_a = 10$ (right).}
\label{hump_formation}
\end{figure}

==> Figures/humpt_formation.tex <==
\begin{figure}[h!]
\centering
% For eps or pdf graphics
\includegraphics[width=0.457\textwidth]{Pictures/current_density.png}\quad
\includegraphics[width=0.457\textwidth]{Pictures/current_density_44.png}
\vspace{-.5cm}
%  \raisebox{1.3in}{a)}\input{figa}\quad
%  \raisebox{1.3in}{b)}\input{figb}
\caption{\small Examples of steady-state solution for different intensities of the magnetic fields, scaled in terms of Hartman number $H_{a} = (\sigma[B]^2U_p/\rho g)^{1/2}$, with $[B]$ the maximum intensity of the magnetic field, $g$ the gravity acceleration(from left to right) and $\sigma$ the electrical conductivity. On the right, the high $H_{a}$ results in a solitary hump in the run-back flow, $H_a = 3$ (left) and $H_a = 10$ (right).}
\label{hump_formation}
\end{figure}

==> Figures/optimization/different_solutions.tex <==
\begin{figure}[H]
\centering\subfloat[Ha = 0.53 \quad $\sigma$ = 16.60]{\label{fig:a}\includegraphics[width=0.45\linewidth]{Pictures/optimization/current_density_0.png}}
\caption{Comparison of the velocity profile sensitivity with respect to $Ha$ at different streamwise locations($\hat{x}$)}
\label{fig:myfig1}
\end{figure}

\begin{figure}[!h]
\centering

\subfloat[Ha = 2.5 \quad $\sigma$ = 8.89]{\label{fig:b}\includegraphics[width=0.45\linewidth]{Pictures/optimization/current_density_1.png}}\\
\subfloat[Ha = 3.74 \quad $\sigma$ = 7.63]{\label{fig:c}\includegraphics[width=0.45\textwidth]{Pictures/optimization/current_density_2.png}}\qquad%
\subfloat[Ha = 7.91 \quad $\sigma$ = 7.29]{\label{fig:d}\includegraphics[width=0.45\textwidth]{Pictures/optimization/current_density_3.png}}%
\caption{Comparison of the velocity profile sensitivity with respect to $Ha$ at different streamwise locations($\hat{x}$)}
\label{fig:myfig1}
\end{figure}

\begin{figure}[!h]
\centering
\subfloat[Ha = 0.53 \quad $\sigma$ = 16.60]{\label{fig:a}\includegraphics[width=0.45\linewidth]{Pictures/optimization/current_density_0.png}}\qquad
\subfloat[Ha = 2.5 \quad $\sigma$ = 8.89]{\label{fig:b}\includegraphics[width=0.45\linewidth]{Pictures/optimization/current_density_1.png}}\\
\subfloat[Ha = 3.74 \quad $\sigma$ = 7.63]{\label{fig:c}\includegraphics[width=0.45\textwidth]{Pictures/optimization/current_density_2.png}}\qquad%
\subfloat[Ha = 7.91 \quad $\sigma$ = 7.29]{\label{fig:d}\includegraphics[width=0.45\textwidth]{Pictures/optimization/current_density_3.png}}%
\caption{Comparison of the velocity profile sensitivity with respect to $Ha$ at different streamwise locations($\hat{x}$)}
\label{fig:myfig1}
\end{figure}

\begin{figure}[!h]
\centering
\subfloat[Ha = 0.53 \quad $\sigma$ = 16.60]{\label{fig:a}\includegraphics[width=0.45\linewidth]{Pictures/optimization/current_density_0.png}}\qquad
\subfloat[Ha = 2.5 \quad $\sigma$ = 8.89]{\label{fig:b}\includegraphics[width=0.45\linewidth]{Pictures/optimization/current_density_1.png}}\\
\subfloat[Ha = 3.74 \quad $\sigma$ = 7.63]{\label{fig:c}\includegraphics[width=0.45\textwidth]{Pictures/optimization/current_density_2.png}}\qquad%
\subfloat[Ha = 7.91 \quad $\sigma$ = 7.29]{\label{fig:d}\includegraphics[width=0.45\textwidth]{Pictures/optimization/current_density_3.png}}%
\caption{Comparison of the velocity profile sensitivity with respect to $Ha$ at different streamwise locations($\hat{x}$)}
\label{fig:myfig1}
\end{figure}

==> Figures/optimization_results.tex <==
\begin{figure}[ht] 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{Pictures/functional_iter_1.png} 
    \caption{} 
    \label{fig7:a} 
    \vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{Pictures/functional_iter_2.png} 
    \caption{} 
    \label{fig7:b} 
    \vspace{4ex}
  \end{subfigure} 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{Pictures/functional_iter_3.png} 
    \caption{} 
    \label{fig7:c} 
  \end{subfigure}%%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{Pictures/functional_iter_4.png} 
    \caption{} 
    \label{fig7:d} 
  \end{subfigure} 
  \caption{Illustration of various images}
  \label{optimization_1} 
\end{figure}

==> Figures/problem_scheme_2.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.4\textwidth]{Pictures/problem_scheme_2.pdf}
    \caption{Schematic of the magnetic wiping with the liquid film over a substrate moving at constant velocity $U_p$, the external magnetic field $B$, the induced current $j$ and the downward Lorentz force $F_L$.}
    \label{problem_scheme_2}
\end{figure}

==> Figures/q_vs_Ha.tex <==
\begin{figure}[h]
\centering
  \begin{center}
    \includegraphics[width=0.5\textwidth]{Pictures/q_vs_Ha.png}
  \end{center}
  \caption{Nondimensional flow rate  $\hat{q}$ as a function of the nondimensional liquid film thickness $\hat{h}$ for different values of the nondimensional magnetic flux $\hat{B}$}
  \label{q_vs_Ha}
\end{figure}

==> Figures/sensitivity_current_1.tex <==
\begin{figure}[!h]
\centering
% For eps or pdf graphics
\includegraphics[width=0.457\textwidth]{Pictures/sensitivity_j_Ha_3_eps_3_1.png}\quad
\includegraphics[width=0.457\textwidth]{Pictures/sensitivity_j_Ha_10_eps_3_1.png}
\vspace{-.5cm}
%  \raisebox{1.3in}{a)}\input{figa}\quad
%  \raisebox{1.3in}{b)}\input{figb}
\caption{Sensitivity of the current density $j(\hat{x},\hat{y})$ with respect to the Hartmann number $Ha$(3(left) and 10(right)) with a Gaussian magnetic field $\hat{B}(\hat{x})$. The horizontal axis reports the nondimensioal stream wise coordinate ($\hat{x}$), the vertical one the value of $\hat{h}(\hat{x})$ and the colours show the gradient}
\label{sensitivity_current_1}
\end{figure}

==> Figures/sensitivity_current_2.tex <==
\begin{figure}[!h]
\centering
% For eps or pdf graphics
\includegraphics[width=0.457\textwidth]{Pictures/sensitivity_j_Ha_3_eps_5_1.png}\quad
\includegraphics[width=0.457\textwidth]{Pictures/sensitivity_j_Ha_10_eps_5_1.png}
\vspace{-.5cm}
%  \raisebox{1.3in}{a)}\input{figa}\quad
%  \raisebox{1.3in}{b)}\input{figb}
\caption{Sensitivity of the current density $j(\hat{x},\hat{y})$ with respect to the Hartmann number $Ha$(3(left) and 10(right)) with a Gaussian magnetic field $\hat{B}(\hat{x})$. The horizontal axis reports the nondimensioal stream wise coordinate ($\hat{x}$), the vertical one the value of $\hat{h}(\hat{x})$ and the colours show the gradient}
\label{sensitivity_current_2}
\end{figure}

==> Figures/sensitivity_velocity_Ha_1.tex <==
\begin{figure}[!h]
\centering
% For eps or pdf graphics
\includegraphics[width=0.457\textwidth]{Pictures/sensitivity_u_Ha_3_eps_3_1.png}\quad
\includegraphics[width=0.457\textwidth]{Pictures/sensitivity_u_Ha_10_eps_3_1.png}
\vspace{-.5cm}
%  \raisebox{1.3in}{a)}\input{figa}\quad
%  \raisebox{1.3in}{b)}\input{figb}
\caption{Sensitivity of the streamwise velocity profile $\hat{u}(\hat{x},\hat{y})$ with respect to the Hartmann number $Ha$(3(left) and 10(right)) with a Gaussian magnetic field $\hat{B}(\hat{x})$  and a standard deviation $\sigma$ = 3. The horizontal axis reports the nondimensioal stream wise coordinate ($\hat{x}$), the vertical one the value of $\hat{h}(\hat{x})$ and the colours show the gradient}
\label{sensitivity_current_1}
\end{figure}

==> Figures/sensitivity_velocity_Ha_2.tex <==
\begin{figure}[!h]
\centering
% For eps or pdf graphics
\includegraphics[width=0.457\textwidth]{Pictures/sensitivity_u_Ha_3_eps_5_1.png}\quad
\includegraphics[width=0.457\textwidth]{Pictures/sensitivity_u_Ha_10_eps_5_1.png}
\vspace{-.5cm}
%  \raisebox{1.3in}{a)}\input{figa}\quad
%  \raisebox{1.3in}{b)}\input{figb}
\caption{Sensitivity of the streamwise velocity profile $\hat{u}(\hat{x},\hat{y})$ with respect to the Hartmann number $Ha$(3(left) and 10(right)) with a Gaussian magnetic field $\hat{B}(\hat{x})$ and a standard deviation $\sigma$=5. The horizontal axis reports the nondimensioal stream wise coordinate ($\hat{x}$), the vertical one the value of $\hat{h}(\hat{x})$ and the colours show the gradient}
\label{sensitivity_current_1}
\end{figure}
